Word Sense Disambiguation with LSTM: Do We Really Need 100 Billion Words?

Recently, Yuan et al. (2016) have shown the effectiveness of using Long Short-Term Memory (LSTM) for performing Word Sense Disambiguation (WSD). Their proposed technique outperformed the previous state-of-the-art with several benchmarks, but neither the training data nor the source code was released. This paper presents the results of a reproduction study of this technique using only openly available datasets (GigaWord, SemCore, OMSTI) and software (TensorFlow). From them, it emerged that state-of-the-art results can be obtained with much less data than hinted by Yuan et al. All code and trained models are made freely available.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}.

% coverage issues
The comparison between all experiments in which we use the MFS-fallback vs all that do not shows that the Precision stays the same or goes down and the recall goes up. The difference is particularly large when we use OMSTI to create the synset embeddings. This is caused by a difference in coverage between SemCor and OMSTI. SemCor contains a relatively low amount of training instances for many unique lemmas, whereas OMSTI contains many training instances for a relatively low amount of training instances.

Last row of Table~\ref{tab:results}



==> implementation.tex <==
\section{Implementation}
\label{sec:implementation}

We extract plain text from Gigaword using the BeautifulSoup HTML parser. We then use the latest English models\footnote{\texttt{en\_core\_web\_md-1.2.1}} of Spacy 1.8.2 to perform sentence boundary detection and tokenization.

The LSTM model is implemented using TensorFlow 1.2.1. We chose TensorFlow because of its industrial-grade quality and because it comes with vital functionalities for training large-scale models.

\subsection{Speeding up training}

The main bottleneck of Yuan et al.'s approach is the training of the LSTM model. Although we do not use a 100-billion word corpus, training the model on Gigaword can still take years if not optimized properly.

To reduce training time, we assume that all (padded) sentences in a training batch have the same length. This simple optimization increases the speed by 17\%. Second, following Yuan et al., we use sampled softmax loss \cite{Jean2014}. Third, we group sentences of similar length together while varying the number of sentences in a batch to fully utilize GPU memory.
%For example, a dataset that contains 5.000 sentences of length 10 and 1.000 sentences of length 50 will be divided into 2 batches, one contains all sentences of length 10 and the other all sentences of length 50. The two batches contain the same number of words. In reality, such a clean division is not possible so we pad shorter sentences to match the length of the longest sentence in its batch. However, thanks to this strategy, the portion of padding symbols decrease from X1-X2\% to around Y\% in all our batches and speed increases by Z times.
Together, the heuristics increase speed by 42 times, making our experiments possible.

\begin{comment}
Optimized batching:

Divided into 49557 batches (63985 elements each, std=100, except last batch of 63945).
Added 74859 elements as padding (0.00%).
Consumed roughly 11.81 GiB.

Stupid batching:

Divided into 157874 batches (63480 elements each, std=2069, except last batch of 63987).
Added 6851449999 elements as padding (68.36%).
Consumed roughly 37.33 GiB.
\end{comment}


